Spectra of quadratic vector fields on $\mathbb{C}^2$: The missing relation

Consider a quadratic vector field on $\mathbb{C}^2$ having an invariant line at infinity and isolated singularities only. We define the extended spectra of singularities to be the collection of the spectra of the linearization matrices of each of the singular points over the affine part, together with all the characteristic numbers (i.e. Camacho-Sad indices) at infinity. This collection consists of 11 complex numbers, and is invariant under affine equivalence of vector fields. In this paper we describe all polynomial relations among these numbers. There are 5 independent polynomial relations; four of them follow from the Euler-Jacobi, the Baum-Bott and the Camacho-Sad index theorems, and are well known. The fifth relation was, until now, completely unknown. We provide an explicit formula for the missing 5th relation, discuss it's meaning and prove that it cannot be formulated as an index theorem.

==> spectraQVFs <==
%%% References for 'invariants' paper

@incollection {BaumBott1970,
    AUTHOR = {Baum, P. and Bott, R.},
     TITLE = {On the zeros of meromorphic vector-fields},
 BOOKTITLE = {Essays on {T}opology and {R}elated {T}opics ({M}\'emoires d\'edi\'es
              \`a {G}eorges de {R}ham)},
     PAGES = {29--47},
 PUBLISHER = {Springer, New York},
      YEAR = {1970},
   MRCLASS = {57.60 (32.00)},
  MRNUMBER = {0261635},
MRREVIEWER = {H. Suzuki},
      NOTE = "\href{http://www.ams.org/mathscinet-getitem?mr=0261635}{MR: 0261635}",
}


@article {CamachoSad1982,
    AUTHOR = {Camacho, C. and Sad, P.},
     TITLE = {Invariant varieties through singularities of holomorphic
              vector fields},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {115},
      YEAR = {1982},
    NUMBER = {3},
     PAGES = {579--595},
      ISSN = {0003-486X},
     CODEN = {ANMAAH},
   MRCLASS = {58F18 (57R99 58A17 58F14)},
  MRNUMBER = {657239 (83m:58062)},
MRREVIEWER = {Robert Roussarie},
       DOI = {10.2307/2007013},
       URL = {http://dx.doi.org/10.2307/2007013},
      NOTE = "\href{http://dx.doi.org/10.2307/2007013}{doi: 10.2307/2007013}",
}


@book {GriffithsHarris1994,
    AUTHOR = {Griffiths, Phillip and Harris, Joseph},
     TITLE = {Principles of algebraic geometry},
    SERIES = {Wiley Classics Library},
 PUBLISHER = {John Wiley \& Sons, Inc., New York},
      YEAR = {1994},
     PAGES = {xiv+813},
      ISBN = {0-471-05059-8},
   MRCLASS = {14-01},
  MRNUMBER = {1288523 (95d:14001)},
       DOI = {10.1002/9781118032527},
       URL = {http://dx.doi.org/10.1002/9781118032527},
      NOTE = "\href{http://dx.doi.org/10.1002/9781118032527}{doi: 10.1002/9781118032527}",
}


@book {Suwa1998,
    AUTHOR = {Suwa, Tatsuo},
     TITLE = {Indices of vector fields and residues of singular holomorphic
              foliations},
    SERIES = {Actualit\'es Math\'ematiques. [Current Mathematical Topics]},
 PUBLISHER = {Hermann, Paris},
      YEAR = {1998},
     PAGES = {viii+204},
      ISBN = {2-7056-6361-4},
   MRCLASS = {32S65 (32L30)},
  MRNUMBER = {1649358},
MRREVIEWER = {M. G. Soares},
      NOTE = "\href{http://www.ams.org/mathscinet-getitem?mr=1649358}{MR: 1649358}",
}


@book {Brunella2015,
    AUTHOR = {Brunella, Marco},
     TITLE = {Birational geometry of foliations},
    SERIES = {IMPA Monographs},
    VOLUME = {1},
 PUBLISHER = {Springer, Cham},
      YEAR = {2015},
     PAGES = {xiv+130},
      ISBN = {978-3-319-14309-5; 978-3-319-14310-1},
   MRCLASS = {14E05 (32C35 32J25 32S65 37F75)},
  MRNUMBER = {3328860},
       DOI = {10.1007/978-3-319-14310-1},
       URL = {https://doi.org/10.1007/978-3-319-14310-1},
      NOTE = "\href{https://doi.org/10.1007/978-3-319-14310-1}{doi: 10.1007/978-3-319-14310-1}",
}


@article {Guillot2004,
    AUTHOR = {Guillot, A.},
     TITLE = {Un th\'eor\`eme de point fixe pour les endomorphismes de
              l'espace projectif avec des applications aux feuilletages
              alg\'ebriques},
   JOURNAL = {Bull. Braz. Math. Soc. (N.S.)},
  FJOURNAL = {Bulletin of the Brazilian Mathematical Society. New Series.
              Boletim da Sociedade Brasileira de Matem\'atica},
    VOLUME = {35},
      YEAR = {2004},
    NUMBER = {3},
     PAGES = {345--362},
      ISSN = {1678-7544},
   MRCLASS = {32S65 (57R25 57R30)},
  MRNUMBER = {2106309 (2006a:32039)},
MRREVIEWER = {M. G. Soares},
       DOI = {10.1007/s00574-004-0018-7},
       URL = {http://dx.doi.org/10.1007/s00574-004-0018-7},
      NOTE = "\href{http://dx.doi.org/10.1007/s00574-004-0018-7}{doi: 10.1007/s00574-004-0018-7}",
}


@article{LinsNeto2012,
    title = {Fibers of the Baum-Bott map for foliations of degree two on {$\mathbb P^2$}},
    volume = {43},
    issn = {1678-7544},
    url = {https://link.springer.com/article/10.1007/s00574-012-0008-0},
    doi = {10.1007/s00574-012-0008-0},
    note = {\href{https://doi.org/10.1007/s00574-012-0008-0}{doi: 10.1007/s00574-012-0008-0}},
    abstract = {The Baum-Bott map associates to a foliation the Baum-Bott indexes of their singularities. In this paper we study the fibers of the Baum-Bott map in the space of foliations of degree two on the projective plane ℙ2. In the main result we prove that its generic fiber contains exactly 240 orbits of the natural action of Aut(ℙ2) onthespace of foliations.},
    pages = {129--169},
    number = {1},
    journal = {Bull Braz Math Soc, New Series},
    author = {Lins Neto, A.},
    urldate = {2017-06-23},
    year = 2012,
    langid = {english},
}


@article{TwinVectorFields,
    AUTHOR = {Ram\'{i}rez, V.},
     TITLE = {Twin vector fields and independence of spectra for quadratic vector fields},
   JOURNAL = {J. Dynam. Control Syst.},
  FJOURNAL = {Journal of Dynamical and Control Systems},
    VOLUME = {23},
      YEAR = {2017},
    NUMBER = {3},
     PAGES = {623--633},
      ISSN = {1079-2724},
   MRCLASS = {37F75},
       DOI = {10.1007/s10883-016-9344-5},
       URL = {http://dx.doi.org/10.1007/s10883-016-9344-5},
      NOTE = "\href{http://dx.doi.org/10.1007/s10883-016-9344-5}{doi: 10.1007/s10883-016-9344-5}",
}


@article{WoodsHole,
    AUTHOR = {Ram\'{i}rez, V.},
     TITLE = {The Woods Hole trace formula and indices for vector fields and foliations on $\mathbb{C}^2$},
   JOURNAL = {\normalfont \href{http://arxiv.org/abs/1608.05321}{arXiv:1608.05321v1} [math.CV]},
      YEAR = {2016},
}


%%% Software


  @Misc{CoCoALib,
   author = {Abbott, J. and Bigatti, A. M.},
   title = {{CoCoALib}: a {C}++ library for doing {C}omputations in {C}ommutative {A}lgebra},
   howpublished = {Available at \url{http://cocoa.dima.unige.it/cocoalib}},
  }
  
  
  @Misc{CoCoA-5,
   author = {Abbott, J. and Bigatti, A. M. and Lagorio, G.},
   title = {{CoCoA-5}: a system for doing {C}omputations in {C}ommutative {A}lgebra},
   howpublished = {Available at \url{http://cocoa.dima.unige.it}},
  }
  
  
@misc {Macaulay2,
    AUTHOR = {Grayson, D. and Stillman, M.},
     TITLE = {Macaulay2, a software system for research in algebraic geometry},
      NOTE = "Available at \url{http://www.math.uiuc.edu/Macaulay2/}"
}


@misc {GiNaC,
      AUTHOR = {{Johannes Gutenberg Universität Mainz}},
       TITLE = {{GiNaC}: A {C}++ library for symbolic computations},
HOWPUBLISHED = {Available at \url{https://www.ginac.de/}},
}


%%% GitHub repository

@misc{GitHubRepo,
  author = {Kudryashov, Yu. and Ramirez, V.},
  title = {Hidden-relation-qvfs},
  publisher = {GitHub},
  howpublished = {GitHub repository. \url{https://github.com/valentermz/Hidden-relation-qvfs}},
  commit = {38cb87f0d5d722b11d8f0c24259eccca2fd7c9aa},
  note = {Commit:~\texttt{38cb87f0d5d7}, 2018}
}

